Cross-Sender Bit-Mixing Coding

Scheduling to avoid packet collisions is a long-standing challenge in networking, and has become even trickier in wireless networks with multiple senders and multiple receivers. In fact, researchers have proved that even {\em perfect} scheduling can only achieve $\mathbf{R} = O(\frac{1}{\ln N})$. Here $N$ is the number of nodes in the network, and $\mathbf{R}$ is the {\em medium utilization rate}. Ideally, one would hope to achieve $\mathbf{R} = \Theta(1)$, while avoiding all the complexities in scheduling. To this end, this paper proposes {\em cross-sender bit-mixing coding} ({\em BMC}), which does not rely on scheduling. Instead, users transmit simultaneously on suitably-chosen slots, and the amount of overlap in different user's slots is controlled via coding. We prove that in all possible network topologies, using BMC enables us to achieve $\mathbf{R}=\Theta(1)$. We also prove that the space and time complexities of BMC encoding/decoding are all low-order polynomials.

==> related-gt-long.tex <==

\section{Group testing}

The notations in the following is not consistent with the remainder of the paper. In the following, $d$ is the number of positives (which corresponds to $k$ in the paper). $N$ is the total number of items (which corresponds to $2^d$ in the paper).

While superimposed code and group testing are closely related, the following subtle difference make superimposed code a somewhat harder problem: In superimposed coding, if the sender uses randomness in its encoding, such randomness will not be directly known to the receiver who needs to decode the message.
Such randomness will then need to be potentially sent to the receiver, in addition to the message itself. In comparison in group testing, encoding and decoding are usually done by a single party, hence avoiding the above problem. This difference implies that certain group testing design that uses a fresh random matrix each time cannot be directly used as practical superimposed code. Our BMC design is for the superimposed code setting, even though it directly applies, without any modification, to the slightly easier group testing setting as well.

\Paragraph{Our unique contribution.}
BMC is a special case of superimposed code~\cite{kautz64}, which in turn is closely related to combinatorial group testing~\cite{du99book}. There has been a large body of work on superimposed code and group testing. To the best of our knowledge, our BMC design is the first superimposed code that {\em simultaneously} has i) polynomial encoding/decoding computational complexity, and ii) $O(d\log N)$ length (which is optimal) independent of $\delta$. Our BMC design also has some other salient features: i) the constant in $O(d\log N)$ is explicit and small --- the length is $9d\log N$, ii) our design is {\em strongly explicit}, in the sense that each codeword can be created (independent from other codewords) in $\mbox{poly}(\log N)$ time and $O(\frac{k}{\delta})$ space. This is in comparison to {\em explicit design}, where a codeword cannot be independently generated and need to be generated together with all other codewords (thus taking $\mbox{poly}(N)$ time). This further contrasts with {\em implicit designs}, where the design only shows the existence of the design, without an explicit way to find such a design.

Many existing designs for superimposed code and group testing follows one of the following two paradigms. The first paradigm is to use a random measurement matrix (e.g., \cite{aldridge14,atia12,chan14,cheraghchi11}). The second paradigm is to use code concatenation (e.g., \cite{bui17,indyk10,lee16,ngo11,vem17}). Here the payload is first encoded into a $q$-ary codeword using some {\em outer code} (e.g., Reed-Solomon code). Next each $q$-ary character in this codeword is individually encoded using some {\em inner code}. There are also some exception. For example, Ngo et al.~\cite{ngo11} uses a recursive design for the code.
Our BMC uses neither random measurement matrix nor code concatenation at all. Rather, we first encode the payload into a codeword using some erasure code. Next we use an LCS to schedule, in a rather fine grained way, the transmission time of each character or bit in this codeword. Hence even though we also use Reed-Solomon code, we leverage its ability to tolerate erasures, and not the minimum distance among its codewords.

\begin{itemize}
\item The first to have optimal number of tests (i.e., $9d\log N = O(d\log N)$), strongly explicit construction, and polynomial decoding time with respect to $d$ and $\log N$. Simple yet elegant design with small constant of $9$.
\item Our approach is rather different from the mainstream approaches for group testing. Two ways to use superimposed code -- to directly send the codeword or to do scheduling -- we use both.
\end{itemize}

\Paragraph{Schemes focusing on efficient encoding/decoding.}
Some other schemes~\cite{bui17,cai17,cheraghchi13,indyk10,lee16,ngo11,vem17} are particularly relevant to us since they aim to both minimize the number of test and also to have efficient encoding/decoding. As a quick summary, all these schemes allow polymonial time encoding/decoding. But none of these achieve the optimal $O(d\log N)$ number tests. The following gives a mode detailed discussion. Indyk et al.~\cite{indyk10} uses concatenated code, with Reed-Solomon code being the outer code, and some independent random binary codes as the inner code. Their design requires
$O(d^2\log N)$ tests. Later Ngo et al.~\cite{ngo11} improves this design by remove certain constraints on $d$, but still using $O(d^2\log N)$ tests. The design in \cite{ngo11} uses concatenated codes, as well as recursive code design. It is worth note that \cite{indyk10,ngo11} do not allow error in decoding.
A lower bound of $\Omega(\frac{d^2}{\log d}\log N)$ is also known~\cite{dyachkov1989superimposed,d1yachkov982bounds}.
%hence their number of tests (i.e., $O(d^2\log N)$) is already optimal~\cite{XXX} under that constraint.


There are also a number of efforts that allow some positive error probability $\delta$ in decoding. (Different works sometime define $\delta$ in different ways, but in all cases, as $\delta$ decreases, the decode results will be closer to the entirely correct results.) Among these efforts, GROTESQUE~\cite{cai17} requires $O(d\log d\log N)$ tests, and relies on random bipartite graphs in its construction. SAFFRON~\cite{lee16} requires $6f(\delta)d\log N$ tests, where $f(\delta)$ is a function of $\delta$ as defined by some optimization problem. In SAFFRON's design, they concatenate sparse-graph codes (as the outer code) with a signature matrix (as the inner code). While $f(\delta)$ has no closed-form, it can be shown that from the optimization problem in \cite{lee16} that $f(\delta)\rightarrow \infty$ as $\delta\rightarrow 0$. This implies that $6f(\delta)d\log N \notin O(d\log N)$, unless we are willing to view $\delta$ as a constant. Bui et al.\cite{bui17} uses  a similar code concatenation approach, and needs $32f(\delta)d\log N$ tests. Vem et al.~\cite{vem17} changes the sparse-graph codes used in SAFFRON, and obtains a design with $f(\delta) d \log \frac{g(\delta)N}{f(\delta)K}$ tests, where $f(\delta)$ and $g(\delta)$ are both functions of $\delta$. They have mainly focused on cases where $\delta$ is viewed as a constant, and did not give an asymptotic bound as a function of $\delta$.

Cheraghchi~\cite{cheraghchi13} proposes a number of schemes while focusing on dealing with noise in the measurement results. For those schemes with polynomial encoding/decoding complexity, the number of tests needed is either $O(d^{3+\alpha + 2/\alpha}\log^{2+2/\alpha} N)$ (for any positive $\alpha$) or $O(d\cdot 2^{\log^3\log N})$, neither of which is within $O(d\log N)$.

%\cite{aldridge14,chan14} admits an error, defined as the probability that the output is not entirely correct (either has false positive or false negative). $O(d\log N)$ tests. Claims to be computationally efficient, but complexity is polynomial with $N$.
%
%\cite{cheraghchi11} admits an error probability, not clearly defined, but seems to be same as \cite{chan14}. Says the error can appraoch zero as $N$ increases. $O(d\log N)$ tests. Claims to be computationally efficient, but complexity is polynomial with $N$.
%
%\cite{sebo85,zhigljavsky03} admits an error probability. $O(d\log N)$ tests. No mention of decoding.
%
%\cite{atia12} admits an error probability. $O(d\log N)$ tests. $N^d$ time decoding.

\Paragraph{Schemes using $O(d\log N)$ tests but not focusing on efficient encoding/decoding.}
Same as our BMC, a number of group testing designs~\cite{aldridge14,atia12,chan14,cheraghchi11,sebo85,zhigljavsky03} in the literature admits some (tunable) probability of error, and requires only $O(d\log N)$ tests. However, these schemes do not provide efficient encoding/decoding algorithms.
Note that some of these works (e.g., \cite{aldridge14,chan14,cheraghchi11}) do mention ``efficient'' encoding/decoding algorithms. However, in their context, ``efficient'' refers to being polynomial with respective to $N$. While our notion of ``efficient'' refers to being polynomial with respective to $\log N$.

\Paragraph{Schemes using $\omega(d\log N)$ tests and not focusing on efficient encoding/decoding.}
There have also been some schemes~\cite{barg17,bui13,cheraghchi09,gilbert12,gilbert08,mazumdar12,mazumdar14,mazumdar16,porat11} that are not explicitly concerned with computationally efficient decoding, even though some of them do allow efficient decoding. (But they may focus on other things such as tolerating more errors.) However, all of these schemes will require $\omega(d\log N)$ tests. Specifically, \cite{barg17} require $O(d\frac{\log^2 N}{\log^2 d})$ tests. \cite{cheraghchi09} requires $O(d^2\log N)$ tests (using random matrices) or $O(d^2\log^2 N)$ tests (using code concatenation).
\cite{mazumdar12,mazumdar16} uses constant-weight code idea, which originated from \cite{kautz64}, but considers not the minimum but the average distance of the codewords. However, these works still cannot achieve $O(d\log N)$ tests. \cite{mazumdar14} uses a random matrix as measurement matrix (also allows certain error in the tests), while requiring $\omega(d\log N)$ tests.

Gilbert et al.~\cite{gilbert12} have proposed two group testing schemes. The first one uses $O(d\log \frac{d}{\delta} \log(\frac{N}{d}\log\frac{d}{\delta}))$ test. The idea is to split the $N$ items into equal-size subsets, where each subset has exactly $\frac{N}{d}\log \frac{d}{\delta}$ items. The scheme will then do group testing on each subset. Their second scheme uses a random measurement matrix and requires $O(d\log\frac{N}{\delta})$ test. Note that the number of tests in neither scheme is within $O(d\log N)$ unless we view $\delta$ as a constant.
Gilbert~\cite{gilbert08} uses random measurement matrices and requires $O(d\log^2 N)$ tests.

Bui et al.~\cite{bui13} requires $O(d^2\log^2 N)$ tests, via code concatenation. Porat and Rothschild's design~\cite{porat11} requires $O(d^2\log N)$ tests, via code concatenation.

\Paragraph{XXX}
\cite{bonis17} uses superimposed code to do scheduling, instead of directly send data. The idea is each node will have a codeword that specifies when the node should access the channel (for example, for sending a data item). The node will then access the channel and transmit the packet in the $i$th interval iff the $i$th bit in the codeword is $1$ (implying that the node may transmit multiple times). Obviously, this will not break the lower bound on general scheduling.


==> wireless-phy-editing.tex <==
Version 2019-01-28:

Todo list:
1) describe the way Glossy achieves time synchronization.

Glossy uses a flooding process to synchronize all the nodes in a network.
The process starts by an initiator node, which transmits a packet carrying a relay counter with value 0.
When a node receives a packet with the relay counter for the first time,
it increments the counter by 1 and immediately reforwards the packet.
Since Glossy makes the software delay between receiving a packet
and reforwarding it a deterministic and network-wide constant,
all neighbors of a sender relay the packet at the same time.
Each forwarding node also records the duration between the start time of the packet it receives
and the start time of the packet it forwards. 
Since all packets being forwarded in a flooding process have the same length, this duration is a network-wide constant too.
Each node can then use the duration length and the relay counter it sees to calculate 
the time that the initiator started the flooding process.
[Glossy]'s experimental result shows that 
Glossy can synchronize neighboring nodes in an IEEE 802.15.4 network 
with a time error smaller than 0.5 mirosecond, which is 
the chip period of IEEE 802.15.4 network.

Potential issues: a worst-case network diameter needs to be assumed.
One round of synchronization can take long... e.g., each pkt is 1ms (the duration measured above),
then it will take 25ms to resync a 25-hop network,
and during this 25ms, the time drift of different nodes (due to their different oscillator) may already be in the range of 0.5us. 
Hence, A faster zippy kind of synchronization method may be needed.

2) 
Question: do we need to add per-symbol preamble / do we need to do re-synchronization in the middle of a BMC round?

For PSK: An oscillator with 20ppm (parts per million) deviates 20 microseconds every second. 
A Zigbee packet of 50 bytes (400bits) lasts less than 2ms, so the deviation is less than 0.04 microseconds in such a packet, 
and resynchronization is not needed.

For BMC, a longer duration for a BMC cycle may be needed. To keep the time drift below 0.5 microsecond, some kind of resynchronization is needed every 25ms. This may be an issue. 


For ASK: different sender's amplitude baseline is different, 
one possibility is to let the receiver recognize (by observing the strength of signals in the first phase, this can be figured out after each sender's code is recognized) and remember each sender's amplitude baseline.
the assumption is that the signal strength remains stable during the whole BMC cycle.

Finally, each symbol contains 32 chips in 802.15.4 protocol. One can imagine we add some pre-agreed chips in the beginning of each symbol as kind of preamble. However, this will make this non-compatible with current protocol.


Section 3.3:

Example systems. While today’s typical modulation schemes do
not explicitly support “blank” bits, “blank” bits are either implementable
or implicitly supported. 

Two examples that may implicitly support BMC are backscatter communication
(e.g., RFID) and OOK modulation (e.g., [Zippy]) systems, which encode “0”
as silence. In such systems, we can simply treat all “blank” bits as
“0” in modulation. 
Achieve bit-level synchronization in these systems is also feasible.
For an RFID system, multiple RFID readers (also called interrogators) can be synchronized 
to sub-microsecond range (e.g., using Precision Time Protocol) through their backhual network.
Once the readers are synchronized, since passive RFID tags communicate by reflecting the incident signal from the readers,
all tags are synchronized as well.

For the OOK modulation based system, [Zippy] implemented a neighborhood synchronization
solution, where an initiator node transmits a single OOK 1 bit, called the synchronization bit. 
The moment a receiver detects the beginning of a synchronization bit,
i.e., by the rising edge of its DATA line, it
immediately transmits a synchronization bit to its own neighborhood. 
As this synchronization process propagates over a multi-hop network, 
all nodes in the network can be synchronized with their neighboring nodes.
[Zippy] shows that using their implementation the per-hop synchronization error is within dozens of microseconds,
which is sufficient for a low-rate network.

Besides backscatter and OOK modulation,
we envision BMC can also be supported by other low-complexity wireless systems (such as LORA) with small modifications.
For example, LORA uses chirp spread spectrum (CSS) modulation, where 
each chirp is a signal whose frequency either increases or decreases with time.
To introduce blank bits into the original LORA design, one possibility is to simply keep
a LORA transceiver silent (i.e., it does not send out any chirp) for the duration of a blank bit.
Depending on the bandwidth and spreading factor used, the duration of a LORA chirp ranges from
hundreds of microseconds to dozens of milliseconds. Hence, the neighborhood synchronization solution
proposed in [Zippy] could likely be applied in a LORA network to help achieve sufficient bit-level synchronization.

The modifications required by BMC on more complex wireless systems will be more involved too.
For example, ZigBee (802.15.4) uses several modulation modes, including DSSS/BPSK, DSSS/O-QPSK, and PSSS/ASK,
where each symbol can carry multiple bits.
One possibility is to introduce blank symbols instead of blank bits for such systems, so as to minimize the changes needed.
This will make BMC's first phase (i.e, the simultaneous transmission of masking strings) less efficient, 
as the duration of a whole symbol is now used to only carry one bit of information.
However, since majority of BMC protocol's air time is spent on the second phase and the second phase can 
use all the bits embedded in each symbol, we expect BMC will still preserve most of its performance advantage.
For systems running at a higher data rate, achieving symbol-level synchronization will also become more challenging.
**
** Insert the description about Glossy's time synchronization approach here **
**
Also, concepts like the guard intervals from OFDM may be needed to help deal with 
imperfect synchronization among nodes.
In fact, for a multi-sender multi-receiver environment, due to the different propagation delays among different sender-receiver pairs,
it is theoretically impossible to achieve perfect synchronization for all of them.




==================

Original text:

Section 1:

Assumptions on physical layer. BMC needs to make certain assumptions
(Section 3.3) on the physical layer. While these assumptions
are already satisfied in certain backscatter communication
systems (e.g., RFID systems) and in systems with OOK modulation,
modifications may be needed in other contexts to satisfy these
assumptions. Since this paper mainly focuses on providing the theoretical
underpinning of our vision, we do not explore further such
modifications. Instead, we hope that our work can attest the great
potential of this direction, and spur future research along this line,
to eventually realize the vision.


Section 3.3:

Example systems. While today’s typical modulation schemes do
not explicitly support “blank” bits, “blank” bits are either implementable
or implicitly supported. For example, backscatter communication
(e.g., RFID systems) and OOK modulation encodes “0”
as silence. In such a case, we can simply treat all “blank” bits as
“0” in modulation. Doing so will directly satisfy all assumptions
above. In other systems, modifications may be needed to satisfy
these assumptions.


==>
Draft of new text:

Section 1:


Assumptions on physical layer. BMC needs to make certain assumptions
(Section 3.3) on the physical layer. While these assumptions
are already satisfied in certain backscatter communication
systems (e.g., RFID systems) and in systems with OOK modulation,
modifications may be needed in other contexts to satisfy these
assumptions. 
We will discuss in Section 3.3 about using BMC with 
example wireless communication technologies
and provide some preliminary suggestions about the potential modifications that could be considered.
We hope that our work can attest the great
potential of this direction and shed some light on the feasibility of doing so, which will spur future research along this line
to eventually realize the vision.


Section 3.3:

Example systems. While today’s typical modulation schemes do
not explicitly support “blank” bits, “blank” bits are either implementable
or implicitly supported. 

Two examples that may implicitly support BMC are backscatter communication
(e.g., RFID) and OOK modulation (e.g., [Zippy]) systems, which encode “0”
as silence. In such systems, we can simply treat all “blank” bits as
“0” in modulation. 
Achieve bit-level synchronization in these systems is also feasible.
For an RFID system, multiple RFID readers (also called interrogators) can be synchronized 
to sub-microsecond range (e.g., using Precision Time Protocol) through their backhual network.
Once the readers are synchronized, since passive RFID tags communicate by reflecting the incident signal from the readers,
all tags are synchronized as well.

For the OOK modulation based system, [Zippy] implemented a neighborhood synchronization
solution, where an initiator node transmits a single OOK 1 bit, called the synchronization bit. 
The moment a receiver detects the beginning of a synchronization bit,
i.e., by the rising edge of its DATA line, it
immediately transmits a synchronization bit to its own neighborhood. 
As this synchronization process propagates over a multi-hop network, 
all nodes in the network can be synchronized with their neighboring nodes.
[Zippy] shows that using their implementation the per-hop synchronization error is within dozens of microseconds,
which is sufficient for a low-rate network.

Besides backscatter and OOK modulation,
we envision BMC can also be supported by other low-complexity wireless systems (such as LORA) with small modifications.
For example, LORA uses chirp spread spectrum (CSS) modulation, where 
each chirp is a signal whose frequency either increases or decreases with time.
To introduce blank bits into the original LORA design, one possibility is to simply keep
a LORA transceiver silent (i.e., it does not send out any chirp) for the duration of a blank bit.
Depending on the bandwidth and spreading factor used, the duration of a LORA chirp ranges from
hundreds of microseconds to dozens of milliseconds. Hence, the neighborhood synchronization solution
proposed in [Zippy] could likely be applied in a LORA network to help achieve sufficient bit-level synchronization.

The modifications required by BMC on more complex wireless systems will be more involved too.
For example, ZigBee (802.15.4) uses several modulation modes, including DSSS/BPSK, DSSS/O-QPSK, and PSSS/ASK,
where each symbol can carry multiple bits.
One possibility is to introduce blank symbols instead of blank bits for such systems, so as to minimize the changes needed.
This will make BMC's first phase (i.e, the simultaneous transmission of masking strings) less efficient, 
as the duration of a whole symbol is now used to only carry one bit of information.
However, since majority of BMC protocol's air time is spent on the second phase and the second phase can 
use all the bits embedded in each symbol, we expect BMC will still preserve most of its performance advantage.
For systems running at a higher data rate, achieving symbol-level synchronization will also become more challenging.
For example, the tens of microsecond synchronization accuracy achieved by [Zippy] may not
be sufficient for ZigBee, where the duration of one symbol can be as low as 16us.
We expect some fine-grained synchronization solutions (see, e.g., [SourceSync]) may be needed here.
Also, concepts like the guard intervals from OFDM may be needed to help deal with 
imperfect synchronization among nodes.
In fact, for a multi-sender multi-receiver environment, due to the different propagation delays among different sender-receiver pairs,
it is theoretically impossible to achieve perfect synchronization for all of them.




